Measurement of the pairwise kinematic Sunyaev-Zeldovich effect with Planck and BOSS data

We present a new measurement of the kinetic Sunyaev-Zeldovich effect (kSZ) using Planck cosmic microwave background (CMB) and Baryon Oscillation Spectroscopic Survey (BOSS) data. Using the `LowZ North/South' galaxy catalogue from BOSS DR12, and the group catalogue from BOSS DR13, we evaluate the mean pairwise kSZ temperature associated with BOSS galaxies. We construct a `Central Galaxies Catalogue' (CGC) which consists of isolated galaxies from the original BOSS data set, and apply the aperture photometry (AP) filter to suppress the primary CMB contribution. By constructing a halo model to fit the pairwise kSZ function, we constrain the mean optical depth to be $\bar{\tau}=(0.53\pm0.32)\times10^{-4}(1.65\,\sigma)$ for `LowZ North CGC', $\bar{\tau}=(0.30\pm0.57)\times10^{-4}(0.53\,\sigma)$ for `LowZ South CGC', and $\bar{\tau}=(0.43\pm0.28)\times10^{-4}(1.53\,\sigma)$ for `DR13 Group'. In addition, we vary the radius of the AP filter and find that the AP size of $7\,{\rm arcmin}$ gives the maximum detection for $\bar{\tau}$. We also investigate the dependence of the signal with halo mass and find $\bar{\tau}=(0.32\pm0.36)\times10^{-4}(0.8\,\sigma)$ and $\bar{\tau}=(0.67\pm0.46)\times10^{-4}(1.4\,\sigma)$ for `DR13 Group' with halo mass restricted to, respectively, less and greater than its median halo mass, $10^{12}\, h^{-1}{\rm M}_{\odot}$. For the `LowZ North CGC' sample restricted to $M_{\rm h} \gtrsim 10^{14}\, h^{-1}{\rm M}_\odot$ there is no detection of the kSZ signal because these high mass halos are associated with the high-redshift galaxies of the LowZ North catalogue, which have limited contribution to the pairwise kSZ signals.

==> table/lowZ_NS_AP_chisq_ap.tex <==
\begin{tabular}{c|cc|cc} \hline\hline
   $\theta_{\rm AP}$&\multicolumn{2}{c|}{LowZ North CGC}
   &\multicolumn{2}{c}{LowZ South CGC} \\

   $[{\rm arcmin}]$
   & $\bar{\tau}[\times10^{-4}]$ & S/N
   & $\bar{\tau}[\times10^{-4}]$ & S/N \\\hline

   $3$
   & $0.39\pm0.25$ & $1.58\sigma$
   & $0.23\pm0.45$ & $0.50\sigma$ \\

   $5$
   & $0.31\pm0.27$ & $1.14\sigma$
   & $0.39\pm0.43$ & $0.90\sigma$ \\

   $7$
   & $0.57\pm0.33$ & $1.71\sigma$
   & $0.33\pm0.59$ & $0.55\sigma$ \\

   $9$
   & $0.38\pm0.40$ & $0.94\sigma$
   & $0.09\pm0.77$ & $0.12\sigma$ \\

   $11$
   & $0.21\pm0.47$ & $0.45\sigma$
   & $-0.05\pm0.91$ & $-0.05\sigma$ \\

   \hline\hline
\end{tabular}


==> table/plot_pkSZ_result_newbin_AP_chisq_ap.tex <==
\begin{tabular}{c|cc|cc|cc} \hline\hline
   $\theta_{\rm AP}$
   &\multicolumn{2}{c|}{LowZ North CGC}
   &\multicolumn{2}{c|}{LowZ South CGC}
   &\multicolumn{2}{c}{DR13 Group} \\

   $[{\rm arcmin}]$
   & $\bar{\tau}[\times10^{-4}]$ & S/N
   & $\bar{\tau}[\times10^{-4}]$ & S/N
   & $\bar{\tau}[\times10^{-4}]$ & S/N \\\hline

   $5$
   & $0.25\pm0.19$ & $1.30\sigma$
   & $0.30\pm0.38$ & $0.79\sigma$
   & $-0.08\pm0.33$ & $-0.23\sigma$ \\

   $6$
   & $0.27\pm0.20$ & $1.34\sigma$
   & $0.41\pm0.28$ & $1.46\sigma$
   & $0.12\pm0.23$ & $0.52\sigma$ \\

   $7$
   & $0.17\pm0.17$ & $0.98\sigma$
   & $0.35\pm0.25$ & $1.43\sigma$
   & $0.38\pm0.16$ & $2.34\sigma$ \\

   $8$
   & $0.20\pm0.15$ & $1.41\sigma$
   & $0.43\pm0.27$ & $1.57\sigma$
   & $0.36\pm0.16$ & $2.24\sigma$ \\

   $9$
   & $0.13\pm0.13$ & $1.03\sigma$
   & $0.06\pm0.20$ & $0.30\sigma$
   & $0.19\pm0.15$ & $1.27\sigma$ \\

   $10$
   & $-0.11\pm0.12$ & $-0.89\sigma$
   & $0.36\pm0.20$ & $1.77\sigma$
   & $0.14\pm0.12$ & $1.14\sigma$ \\

   $11$
   & $0.06\pm0.11$ & $0.50\sigma$
   & $0.62\pm0.17$ & $3.68\sigma$
   & $0.03\pm0.11$ & $0.24\sigma$ \\

   \hline\hline
\end{tabular}


==> table/plot_pkSZ_result_newbin_JK_AP_chisq_ap.tex <==
\begin{tabular}{c|cc|cc|cc} \hline\hline
   $\theta_{\rm AP}$
   &\multicolumn{2}{c|}{LowZ North CGC}
   &\multicolumn{2}{c|}{LowZ South CGC}
   &\multicolumn{2}{c}{DR13 Group} \\

   $[{\rm arcmin}]$
   & $\bar{\tau}[\times10^{-4}]$ & S/N
   & $\bar{\tau}[\times10^{-4}]$ & S/N
   & $\bar{\tau}[\times10^{-4}]$ & S/N \\\hline

   $5$
   & $0.52\pm0.20$ & $2.65\sigma$
   & $0.22\pm0.35$ & $0.64\sigma$
   & $0.07\pm0.27$ & $0.28\sigma$ \\

   $6$
   & $0.52\pm0.22$ & $2.40\sigma$
   & $0.19\pm0.39$ & $0.48\sigma$
   & $0.14\pm0.33$ & $0.42\sigma$ \\

   $7$
   & $0.60\pm0.28$ & $2.15\sigma$
   & $-0.18\pm0.45$ & $-0.41\sigma$
   & $0.56\pm0.31$ & $1.84\sigma$ \\

   $8$
   & $0.53\pm0.32$ & $1.64\sigma$
   & $-0.05\pm0.50$ & $-0.11\sigma$
   & $0.66\pm0.32$ & $2.08\sigma$ \\

   $9$
   & $0.38\pm0.35$ & $1.08\sigma$
   & $-0.03\pm0.56$ & $-0.05\sigma$
   & $0.60\pm0.33$ & $1.84\sigma$ \\

   $10$
   & $0.26\pm0.37$ & $0.69\sigma$
   & $0.04\pm0.56$ & $0.08\sigma$
   & $0.55\pm0.33$ & $1.64\sigma$ \\

   $11$
   & $0.11\pm0.38$ & $0.28\sigma$
   & $0.16\pm0.51$ & $0.32\sigma$
   & $0.58\pm0.35$ & $1.65\sigma$ \\

   \hline\hline
\end{tabular}


==> table/plot_pkSZ_result_newbin_all_AP_chisq_ap.tex <==
\begin{tabular}{c|cc|cc|cc} \hline\hline
   $\theta_{\rm AP}$
   &\multicolumn{2}{c|}{LowZ North CGC}
   &\multicolumn{2}{c|}{LowZ South CGC}
   &\multicolumn{2}{c}{DR13 Group} \\

   $[{\rm arcmin}]$
   & $\bar{\tau}[\times10^{-4}]$ & S/N
   & $\bar{\tau}[\times10^{-4}]$ & S/N
   & $\bar{\tau}[\times10^{-4}]$ & S/N \\\hline

   $5$
   & $0.12\pm0.18$ & $0.70\sigma$
   & $0.19\pm0.28$ & $0.68\sigma$
   & $0.11\pm0.21$ & $0.52\sigma$ \\

   $6$
   & $0.04\pm0.17$ & $0.23\sigma$
   & $0.39\pm0.20$ & $1.97\sigma$
   & $0.13\pm0.23$ & $0.55\sigma$ \\

   $7$
   & $0.26\pm0.20$ & $1.31\sigma$
   & $0.25\pm0.29$ & $0.86\sigma$
   & $0.38\pm0.29$ & $1.31\sigma$ \\

   $8$
   & $0.14\pm0.23$ & $0.61\sigma$
   & $0.50\pm0.31$ & $1.60\sigma$
   & $0.28\pm0.31$ & $0.92\sigma$ \\

   $9$
   & $-0.06\pm0.27$ & $-0.22\sigma$
   & $0.39\pm0.46$ & $0.86\sigma$
   & $0.13\pm0.32$ & $0.41\sigma$ \\

   $10$
   & $-0.09\pm0.30$ & $-0.29\sigma$
   & $0.42\pm0.53$ & $0.80\sigma$
   & $0.08\pm0.32$ & $0.25\sigma$ \\

   $11$
   & $-0.02\pm0.34$ & $-0.07\sigma$
   & $0.03\pm0.58$ & $0.04\sigma$
   & $0.18\pm0.33$ & $0.56\sigma$ \\

   \hline\hline
\end{tabular}


==> table/written_table.tex <==
\centering
\begin{tabular}{c|cc|cc} \hline\hline
& \multicolumn{2}{|c}{LowZ North CGC}& \multicolumn{2}{|c}{DR13 Group}\\
\hline
Parameter & Best fit & $68\%$ limits& Best fit & $68\%$ limits\\
\hline
$z_{\rm eff}$  & $  0.1488$ & $  0.1063_{ -0.0180 -0.0614}^{+  0.2380+  0.3245}$ & $  0.0534$ & $  0.0604_{ -0.0153 -0.0411}^{+  0.2583+  0.3683}$ \\
$\log M_{\rm h}$  & $ 13.2356$ & $ 13.3156_{ -0.4743 -1.5733}^{+  0.3764+  2.1184}$ & $ 12.5811$ & $ 12.6877_{ -1.3337 -2.4566}^{+  1.7687+  3.1282}$ \\
\hline\hline
\end{tabular}

